On the Power of Statistical Zero Knowledge

We examine the power of statistical zero knowledge proofs (captured by the complexity class SZK) and their variants. First, we give the strongest known relativized evidence that SZK contains hard problems, by exhibiting an oracle relative to which SZK (indeed, even NISZK) is not contained in the class UPP, containing those problems solvable by randomized algorithms with unbounded error. This answers an open question of Watrous from 2002 [Aar]. Second, we "lift" this oracle separation to the setting of communication complexity, thereby answering a question of G\"o\"os et al. (ICALP 2016). Third, we give relativized evidence that perfect zero knowledge proofs (captured by the class PZK) are weaker than general zero knowledge proofs. Specifically, we exhibit oracles relative to which SZK is not contained in PZK, NISZK is not contained in NIPZK, and PZK is not equal to coPZK. The first of these results answers a question raised in 1991 by Aiello and H{\aa}stad (Information and Computation), and the second answers a question of Lovett and Zhang (2016). We also describe additional applications of these results outside of structural complexity. The technical core of our results is a stronger hardness amplification theorem for approximate degree, which roughly says that composing the gapped-majority function with any function of high approximate degree yields a function with high threshold degree.

==> app_otheroracleseps.tex <==
\section{$\PZK$ vs $\coPZK$}
\label{sec:others2}
\label{sec:copzk}

In order to prove Theorem~\ref{thm:pzk-copzk}, we first show that $\HVPZK$ is closed under ``composition'' with $\mathsf{GapAND}$.

\begin{lemma}
    \label{lem:pzk-closure}
    Let $f:D \to \{0,1\}$ with $D \in \{0,1\}^M$ be a partial function and $n$ be a positive integer, $1/2 < \epsilon < 1$ be a constant. If $f$ has a $\polylog(M)$-time $\HVPZK$ protocol, then $\GapAND{f}{n}{\epsilon}$ has a $\polylog(nM)$-time $\HVPZK$ protocol.
\end{lemma}

\begin{proof}
    For convenience, denote $\GapAND{f}{n}{\epsilon}$ by $g$. Given an $\HVPZK$ protocol $(P,V,S)$ for $f$, we will construct an $\HVPZK$ protocol $(P',V',S')$ for $g$. Given an input $x = (x_1, \dots, x_n)$ for $g$, $V'$ selects, say, $\log^2(n)$ values of $i \in [n]$, and $P'$ and $V'$ run the interactive protocol $(P,V)$ on each of the corresponding $x_i$'s independently. $V'$ accepts if and only if $(P,V)$ accepts on all these $x_i$'s. Completeness and soundness follows easily from standard arguments and the definition of $g$.

    On a similar input, the simulator $S'$ simply selects the same number of $i$'s, and runs $S$ on the corresponding $x_i$'s. Since in a YES instance all of the $x_i$'s are such that $f(x_i) = 1$, $S$ simulates the transcripts of $(P,V)$ on all of these exactly, except with a negligible probability when it fails on one or more of these. Hence $S'$ simulates $(P',V')$ exactly as well, again failing only with a negligible probability.
\end{proof}

We will need the following implication of the constructions in~\cite{DGOW95}.

\begin{lemma}[Implied by \cite{DGOW95}]
    \label{lem:nipzk-pzk}
    Any partial Boolean function that has a $\polylog(n)$-time $\NIPZK$ protocol also has a $\polylog(n)$-time $\PZK$ protocol.
\end{lemma}

We will use the function $\PTP_n$ (cf. Definition~\ref{defi:ptp}) to establish our separation. The following are immediate consequences of Theorems~\ref{theo:ptp} and \ref{theo:lift-UPP} and Lemma~\ref{lm:dega-to-ppdt}.
\begin{cor}
    \label{cor:ptp}
      $\PPdt(\GapAND{\overline{\PTP}_n}{n}{7/8}) = \Omega(n^{1/3})$
\end{cor}

\begin{lemma}
    \label{lem:ptp-pzk}
    $\PTP_n$ has a $\polylog(n)$-time $\PZK$ protocol.
\end{lemma}

\begin{proof}
    We will show this by presenting a $\polylog(n)$-time $\NIPZK$ protocol for $\PTP_n$ and invoking Lemma~\ref{lem:nipzk-pzk}. The protocol is very similar to the one described in Section \ref{sec:ptpprotocol}. Given a function $f:[n]\rightarrow [n]$ as input, an $r\in [n]$ is chosen at random using the common random string. $P$ is then supposed to send an $x$ to $V$ such that $f(x) = r$. $V$ accepts if this is true. Completeness, soundness and perfect zero-knowledge are all easily argued using the definition of $\PTP_n$.
\end{proof}

Now we have everything we need to prove Theorem~\ref{thm:pzk-copzk}, which we repeat below.

\begin{theo}[]
    \label{thm:pzk-copzk-again}
    There is an oracle $\Oracle$ such that $\PZK^\Oracle \neq \co\PZK^\Oracle$.
\end{theo}

\begin{proof}
    Suppose $\PZK^\Oracle = \coPZK^\Oracle$ with respect to all oracles $\Oracle$. This implies that any language that is in $\polylog(n)$-time $\PZK$ is also in $\polylog(n)$-time $\coPZK$, and vice versa -- if this were not true for some language, then we would be able to use that language to construct an oracle that separates the two classes by diagonalization. In particular, this hypothesis and Lemma~\ref{lem:ptp-pzk} imply that $\overline{\PTP}_n$ has a $\polylog(n)$-time $\PZK$ (and hence $\HVPZK$) protocol. Then, by Lemma~\ref{lem:pzk-closure}, $\GapAND{\overline{\PTP}_n}{n}{7/8}$ has a $\polylog(n)$-time $\HVPZK$ protocol.

    This fact, along with the lower bound in Corollary~\ref{cor:ptp}, can be used to construct an oracle separating $\HVPZK$ from $\PP$ by standard diagonalization. But by Lemma~\ref{lem:pzk-pp}, such an oracle cannot exist. So there has to be some oracle separating $\PZK$ and $\coPZK$. 
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 
